Fluid statics of a self-gravitating perfect-gas isothermal sphere

We open the paper with introductory considerations describing the motivations of our long-term research plan targeting gravitomagnetism, illustrating the fluid-dynamics numerical test case selected for that purpose, that is, a perfect-gas sphere contained in a solid shell located in empty space sufficiently away from other masses, and defining the main objective of this study: the determination of the gravitofluid-static field required as initial field ($t=0$) in forthcoming fluid-dynamics calculations. The determination of the gravitofluid-static field requires the solution of the isothermal-sphere Lane-Emden equation. We do not follow the habitual approach of the literature based on the prescription of the central density as boundary condition; we impose the gravitational field at the solid-shell internal wall. As the discourse develops, we point out differences and similarities between the literature's and our approach. We show that the nondimensional formulation of the problem hinges on a unique physical characteristic number that we call gravitational number because it gauges the self-gravity effects on the gas' fluid statics. We illustrate and discuss numerical results; some peculiarities, such as gravitational-number upper bound and multiple solutions, lead us to investigate the thermodynamics of the physical system, particularly entropy and energy, and preliminarily explore whether or not thermodynamic-stability reasons could provide justification for either selection or exclusion of multiple solutions. We close the paper with a summary of the present study in which we draw conclusions and describe future work.

==> myrgreekmacros.tex <==
% requires  rgreekmacros.tex; available only at 10pt (I believe)

\newcommand{\greekdg}[1]{\mbox{\begingreek#1\endgreek}}
\newcommand{\mgreekdg}[1]{\mbox{\beginmgreek#1\endmgreek}}

\newcommand{\alphay}{\mgreekdg{a}} 

\newcommand{\betay}{\mgreekdg{b}}

\newcommand{\gammay}{\mgreekdg{g}}

\newcommand{\deltay}{\mgreekdg{d}}
  \newcommand{\sdeltay}{\mgreekdg{\small d}}

\newcommand{\varepsilony}{\large \mgreekdg{e}}

\newcommand{\etay}{\mgreekdg{h}}
   \newcommand{\obetay}{\bar{\etay}}   % over-barred etay
   \newcommand{\setay}{\scalebox{0.80}{\etay}} % sub/superscript etay
   \newcommand{\etayA}{\etay_{\scalebox{0.5}{A}}}
%   \newcommand{\setayA}{\scalebox{0.825}{$\etayA$}} % sub/superscript etayA     
   \newcommand{\setayA}{{\setay}_{\scalebox{0.45}{A}}}
   \newcommand{\etayAa}{\etay_{\scalebox{0.5}{A,$a$}}}
   \newcommand{\setayAa}{{\setay}_{\scalebox{0.45}{A,$a$}}}
   \newcommand{\etayE}{\etay_{\scalebox{0.5}{E}}}
   \newcommand{\etayEa}{\etay_{\scalebox{0.5}{E,$a$}}}
   \newcommand{\etayK}{\etay_{\scalebox{0.5}{K}}}
   \newcommand{\etayKa}{\etay_{\scalebox{0.5}{K,$a$}}}

\newcommand{\thetay}{\mgreekdg{j}}

\newcommand{\iotay}{\mgreekdg{i}}

\newcommand{\ky}{\mgreekdg{k}}
   \newcommand{\kyb}{\mgreekdg{\bf k}}
   \newcommand{\kys}{\mgreekdg{\sl k}}

\newcommand{\lambday}{\mgreekdg{l}}
   \newcommand{\lambdayb}{\mgreekdg{\bf l}}
   \newcommand{\lambdays}{\mgreekdg{\sl l}}

\newcommand{\muy}{\mgreekdg{m}}
   \newcommand{\lmuy}{\mgreekdg{\large m}}
   \newcommand{\muyb}{\mgreekdg{\bf m}}

\newcommand{\nuy}{\mgreekdg{n}}

\newcommand{\xiy}{\mgreekdg{x}}
   \newcommand{\xiyA}{\xiy_{\scalebox{0.5}{A}}}
   \newcommand{\xiyE}{\xiy_{\scalebox{0.5}{E}}}
   \newcommand{\xiyK}{\xiy_{\scalebox{0.5}{K}}}
      
\newcommand{\piy}{\mgreekdg{p}}

\newcommand{\rhoy}{\mgreekdg{r}}
   \newcommand{\brhoy}{\bar{\rhoy}}
   \newcommand{\trhoy}{\tilde{\rhoy}}
   \newcommand{\trhoyA}{\tilde{\rhoy}_{\scalebox{0.5}{A}}}
   \newcommand{\trhoyE}{\tilde{\rhoy}_{\scalebox{0.5}{E}}}
   \newcommand{\trhoyK}{\tilde{\rhoy}_{\scalebox{0.5}{K}}}
   \newcommand{\rhoyc}{\rhoy_{\ssub{.6}{0}}}
   
\newcommand{\sigmay}{\mgreekdg{s}}
   \newcommand{\sigmayb}{\mgreekdg{\bf s}}

\newcommand{\tauy}{\mgreekdg{t}}

\newcommand{\phiy}{\mgreekdg{f}}

\newcommand{\psiy}{\mgreekdg{y}}


\newcommand{\Piy}{\mgreekdg{P}}
  \newcommand{\tPiy}{\tiny \mgreekdg{P}}

\newcommand{\Phiyb}{\mgreekdg{\bf F}}





==> rgreekmacros.tex <==
\def\lt{<}
\def\gt{>}
\newcount\fontnumber
\fontnumber=0
\newif\ifoneaccent\oneaccenttrue
\def\ifnextchar#1#2#3{\let\tempe #1\def\tempa{#2}\def\tempb{#3}\futurelet
  \tempc\ifnch}
\def\ifnch{\ifx\tempc\tempe\let\tempd\tempa\else\let\tempd\tempb\fi\tempd}
\def\gobble#1{}
\def\greekmode{%
\catcode`\<=13%
\catcode`\>=13%
\catcode`\'=11%
\catcode`\`=13%
\catcode`\~=11%
\catcode`\"=13%
\lccode`\<=`\<%
\lccode`\>=`\>%
\lccode`\'=`\'%
\lccode`\~=`\~%
\lccode`\"=`\"%
\def\rg{\fontnumber=1\tengr}%
\def\sl{\fontnumber=2\tengrsl}%
\def\it{\fontnumber=3\tengrit}%
\def\bf{\fontnumber=4\tengrbf}%
\def\smc{\fontnumber=5\tengrsmc}%
\def\I##1{\setbox0\hbox{##1}\ifdim\ht0=1ex\accent'174 ##1%
  \else{\ooalign{\hidewidth\char'174\hidewidth\crcr\unhbox0}}\fi}}%
\newcount\vwl
\newcount\acct
{
  \greekmode
  \gdef>{\ifnextchar ~{\expandafter\smoothcircumflex\gobble}{\char\lq\>}}
  \gdef<{\ifnextchar ~{\expandafter\roughcircumflex\gobble}{\char\lq\<}}
  \gdef\smoothcircumflex#1{\acct=\rq134 \vwl=\lq#1 \dobreathingcircumflex}
  \gdef\roughcircumflex#1{\acct=\rq100 \vwl=\lq#1 \dobreathingcircumflex}
  \gdef\dobreathingcircumflex{\ifnum\vwl\lt\rq140 %if uppercase
    \char\the\acct\kern -.2em\char\the\vwl\else
    \doaccent\fi}
  \gdef\doaccent{\accent\the\acct \char\the\vwl\relax}
  \gdef"{\ifnextchar '{\expandafter\diaeresisacute\gobble}{\accent\lq\"}}
  \gdef\diaeresisacute#1{\accent\rq043 #1}
  \gdef`{'}
}
 
\newif\ifgreek\greekfalse
 
\def\begingreek{\bgroup\font\tengr=rgrrg10\font\tengrsl=rgrsl10%
\font\tengrbf=rgrbf10\font\tengrit=rgrti10\font\tengrsmc=rgrsc10%
\greektrue\greekmode\rg}
\def\beginmgreek{\bgroup\font\tengr=mrgrrg10\font\tengrsl=mrgrsl10%
\font\tengrbf=mrgrbf10\font\tengrit=mrgrti10\font\tengrsmc=rgrsc10%
\greektrue\greekmode\rg}
\def\endgreek{\egroup}
\def\endmgreek{\egroup}
\def\monotoniko{%
\font\tengr=mrgrrg10\font\tengrsl=mrgrsl10%
\font\tengrbf=mrgrbf10\font\tengrit=mrgrti10%
\ifnum\fontnumber=5\smc%
  \else\ifnum\fontnumber=4\bf%
    \else\ifnum\fontnumber=3\it%
      \else\ifnum\fontnumber=2\sl%
        \else\rg%
      \fi%
    \fi%
  \fi%
\fi%
}
\def\polutoniko{%
\font\tengr=rgrrg10\font\tengrsl=rgrsl10%
\font\tengrbf=rgrbf10\font\tengrit=rgrti10%
\ifnum\fontnumber=5\smc%
  \else\ifnum\fontnumber=4\bf%
    \else\ifnum\fontnumber=3\it%
      \else\ifnum\fontnumber=2\sl%
        \else\rg%
      \fi%
    \fi%
  \fi%
\fi%
}
\let\math=$%
{\catcode`\$=13%
\gdef\greekdelims{\catcode`\$=13%
\def${\ifgreek\endgreek\else\begingreek\fi}
\def\display{\math\math}\def\enddisplay{\math\math}}}
\def\grave#1{{\edef\next{\the\font}\smc\accent\rq001\next#1}}
\def\roughgrave#1{{\edef\next{\the\font}\smc\accent\rq002\next#1}}
\def\smoothgrave#1{{\edef\next{\the\font}\smc\accent\rq003\next#1}}
\def\diaeresisgrave#1{{\edef\next{\the\font}\smc\accent\rq004\next#1}}
\def\diaeresiscircumflex#1{{\edef\next{\the\font}\smc\accent\rq005\next#1}}
\def\breve#1{{\edef\next{\the\font}\smc\accent\rq006\next#1}}
\def\macron#1{{\edef\next{\the\font}\smc\accent\rq007\next#1}}
\def\rhorough{{\tengrsmc
\ifnum\fontnumber=5\char\rq162
  \else\ifnum\fontnumber=4\char\rq016
    \else\ifnum\fontnumber=3\char\rq014
      \else\ifnum\fontnumber=2\char\rq012
        \else\char\rq010
      \fi
    \fi
  \fi
\fi
}}
\def\rhosmooth{{\tengrsmc
\ifnum\fontnumber=5\char\rq162
  \else\ifnum\fontnumber=4\char\rq017
    \else\ifnum\fontnumber=3\char\rq015
      \else\ifnum\fontnumber=2\char\rq013
        \else\char\rq011
      \fi
    \fi
  \fi
\fi
}}
\def\digamma{{\smc\char\rq135}}
\def\smallDigamma{{\smc\char\rq140}}
\def\Digamma{{\tengrsmc
\ifnum\fontnumber=5\char\rq021
  \else\ifnum\fontnumber=4\char\rq027
    \else\ifnum\fontnumber=3\char\rq025
      \else\ifnum\fontnumber=2\char\rq023
        \else\char\rq021
      \fi
    \fi
  \fi
\fi
}}
\def\vardigamma{{\tengrsmc
\ifnum\fontnumber=5\char\rq020
  \else\ifnum\fontnumber=4\char\rq026
    \else\ifnum\fontnumber=3\char\rq024
      \else\ifnum\fontnumber=2\char\rq022
        \else\char\rq020
      \fi
    \fi
  \fi
\fi
}}
\def\understroke{{\smc\char\rq046}}
\def\overstroke{{\smc\char\rq044}}
\def\sanpi{{\smc\char\rq136}}
\def\Sanpi{{\smc\char\rq137}}
\def\qoppa{{\smc\char\rq133}}
\def\varqoppa{{\smc\char\rq134}}
\def\Qoppa{{\smc\char\rq103}}
\def\Tao{{\smc\char\rq177}}
\def\ssh{\breve{s}}\def\SSH{\breve{S}}
\def\dz{\breve{z}}\def\DZ{\breve{Z}}
\def\psh{\breve{y}}\def\PSH{\breve{Y}}
\def\ksh{\breve{x}}\def\KSH{\breve{X}}
\def\inviota{{\smc\char\rq126}}
\def\grMF{{\smc\char\rq030\char\rq031\char\rq032\char\rq033}\-{\smc%
\char\rq034\char\rq036\char\rq037\char\rq032}}
\def\MF{{\smc\char\rq030\char\rq031\char\rq032\char\rq033}\-{\smc%
\char\rq040\char\rq036\char\rq037\char\rq032}}
 
\endinput
 

